Reasoning about Regular Properties: A Comparative Study

Several new algorithms for deciding emptiness of Boolean combinations of regular languages and of languages of alternating automata (AFA) have been proposed recently, especially in the context of analysing regular expressions and in string constraint solving. The new algorithms demonstrated a significant potential, but they have never been systematically compared, neither among each other nor with the state-of-the art implementations of existing (non)deterministic automata-based methods. In this paper, we provide the first such comparison as well as an overview of the existing algorithms and their implementations. We collect a diverse benchmark mostly originating in or related to practical problems from string constraint solving, analysing LTL properties, and regular model checking, and evaluate collected implementations on it. The results reveal the best tools and hint on what the best algorithms and implementation techniques are. Roughly, although some advanced algorithms are fast, such as antichain algorithms and reductions to IC3/PDR, they are not as overwhelmingly dominant as sometimes presented and there is no clear winner. The simplest NFA-based technology may be actually the best choice, depending on the problem source and implementation style. Our findings should be highly relevant for development of these techniques as well as for related fields such as string constraint solving.

==> figs/a-stats-mean-only.tex <==
 tool        & \multicolumn{2}{c}{a-ltlf}   & \multicolumn{2}{c}{a-param}   & \multicolumn{2}{c}{a-rand}   & \multicolumn{2}{c}{a-sloth}   & \multicolumn{2}{c}{a-spag}   & \multicolumn{2}{c}{a-spec}   \\
\hline
 \abc        & \win{0.1} & \win{0}          & 25.4 & 134                    & \win{0.1} & \win{0}          & \win{1.3} & 34                & \win{0.2} & \win{1}          & \win{0.1} & \win{0}          \\
 \jaltimpact & \win{4.0} & \win{0}          & 47.0 & 205                    & \win{7.9} & 12               & 24.9 & 1005                   & \win{5.7} & 130              & \win{2.4} & \win{0}          \\
 \minisat    & 31.0 & 868                   & 58.3 & 310                    & 18.3 & 84                    & 14.8 & 978                    & \win{1.0} & 46               & \win{0.0} & \win{0}          \\
 \bisim      & 37.0 & 1013                  & 58.2 & 308                    & \win{4.4} & \win{8}          & 17.5 & 1087                   & 21.6 & 992                   & 32.9 & 32                    \\
\hline

==> figs/b-stats-mean-only.tex <==
 tool        & \multicolumn{2}{c}{b-hand}   & \multicolumn{2}{c}{b-incl}   & \multicolumn{2}{c}{b-param}   & \multicolumn{2}{c}{b-rex}   & \multicolumn{2}{c}{b-smt}   \\
\hline
 \jaltimpact & 11.1 & \win{5}               & 30.0 & 28                    & 57.8 & 252                    & 12.2 & 48                   & \win{3.5} & \win{0}         \\
 \minisat    & \win{1.4} & \win{1}          & 43.7 & 55                    & 39.0 & 147                    & \win{9.3} & 45              & \win{0.0} & \win{0}         \\
 \bisim      & 11.2 & \win{8}               & 14.1 & 15                    & 55.4 & 240                    & \win{3.8} & 15              & \win{2.5} & \win{0}         \\
 \dotnet     & \win{0.2} & \win{0}          & \win{3.4} & \win{0}          & 46.3 & 161                    & \win{0.2} & \win{0}         & \win{0.2} & \win{0}         \\
 \mona       & 27.3 & 22                    & 33.0 & 33                    & 44.9 & 25                     & 41.0 & 15                   & \win{1.5} & \win{8}         \\
 \ours       & \win{0.1} & \win{0}          & \win{3.0} & \win{0}          & 46.5 & 204                    & \win{0.5} & \win{0}         & \win{0.0} & \win{0}         \\
 \vata       & \multicolumn{2}{c|}{-}       & \win{3.2} & \win{0}          & \multicolumn{2}{c|}{-}        & \win{2.1} & 10              & \multicolumn{2}{c}{-}      \\
 \abc        & \win{0.4} & \win{0}          & \win{4.8} & \win{1}          & 44.9 & 191                    & \win{0.2} & \win{0}         & \win{0.1} & \win{0}         \\
 \cvc        & 27.4 & 10                    & \multicolumn{2}{c|}{-}       & 48.6 & 208                    & \multicolumn{2}{c|}{-}      & \win{0.8} & \win{1}         \\
 \zthree     & \win{3.9} & \win{2}          & \multicolumn{2}{c|}{-}       & 32.0 & 129                    & \multicolumn{2}{c|}{-}      & \win{0.4} & \win{2}         \\
 \brics      & \win{3.9} & \win{3}          & \multicolumn{2}{c|}{-}       & 52.7 & 228                    & \win{5.8} & 40              & \win{0.3} & \win{0}         \\
\hline

